Optimal Resource Allocation with Delay Guarantees for Network Slicing in Disaggregated RAN

In this article, we propose a novel formulation for the resource allocation problem of a sliced and disaggregated Radio Access Network (RAN) and its transport network. Our proposal assures an end-to-end delay bound for the Ultra-Reliable and Low-Latency Communication (URLLC) use case while jointly considering the number of admitted users, the transmission rate allocation per slice, the functional split of RAN nodes and the routing paths in the transport network. We use deterministic network calculus theory to calculate delay along the transport network connecting disaggregated RANs deploying network functions at the Radio Unit (RU), Distributed Unit (DU), and Central Unit (CU) nodes. The maximum end-to-end delay is a constraint in the optimization-based formulation that aims to maximize Mobile Network Operator (MNO) profit, considering a cash flow analysis to model revenue and operational costs using data from one of the world's leading MNOs. The optimization model leverages a Flexible Functional Split (FFS) approach to provide a new degree of freedom to the resource allocation strategy. Simulation results reveal that, due to its non-linear nature, there is no trivial solution to the proposed optimization problem formulation. Our proposal guarantees a maximum delay for URLLC services while satisfying minimal bandwidth requirements for enhanced Mobile BroadBand (eMBB) services and maximizing the MNO's profit.

==> Tables/Parameters.tex <==
\begin{table}[htb]
	\centering
\begin{threeparttable}
	\caption{Parameters}
    \label{tab:parameters}

	\begin{tabular}{|l|l|l|}
		\hline
		Parameter & $R$ (Mbps) & $T\tnote{1}$ ($\mu$s)\\
		\hline\rowcolor{Gray}
		node 1 (vDU) & 50 & 40.96  \\
		\hline
            node 2 (eth) & 100 & 40.96  \\
		\hline\rowcolor{Gray}
		node 3 (ring) & 250 & 36.384 \\
		\hline
		node 4 (ring) & 250 & 28.192  \\
		\hline\rowcolor{Gray}
		node 5 (ring) & 250 & 24.096  \\
            \hline
		\hline
		Parameter & $\rho$ (kbps) & $\sigma$ (bits)  \\
            \hline\rowcolor{Gray}
		URLLC  & 1024  & 1024  \\
		\hline
		eMBB  & 2048  &  2048  \\
            \hline
	\end{tabular}
 \begin{tablenotes}
   \item[1] This value already takes into account PD (Propagation Delay).  
  \end{tablenotes}
  \end{threeparttable}
\end{table}

==> Tables/Parameters1.tex <==
\begin{table}[htb]
	\centering
\begin{threeparttable}
	\caption{Parameters for Simulation with URLLC flows and Bundled Option (D-RAN) as the O-RAN scenario (see subsection \ref{subsection:O-ran}).}
           \label{Tab:Parameters1}
	\begin{tabular}{|c|c|c|}
		\hline
		Parameter & $R$ (Mbps) & $T\tnote{1}$ ($\mu$s) \\
		\hline
		vDU & 150 & $L_{max}*8/150$  \\
		\hline
            eth & 1000 & $L_{max}*8/1000$   \\
		\hline
		ring & 2500 & $L_{max}*8/2500$   \\
		  \hline
		\hline
		Parameter & $\rho$ (bps) & $\sigma$ (bits)\\
            \hline
		flow  & $1024\times 10^3$ & 1024 \\
		\hline
	\end{tabular}
 \begin{tablenotes}
   \item[1] This value is obtained using $T=\frac{L_{max}*8}{R}$. For URLLC, we considered a packet size of $L_{max}$=128 Bytes.  
  \end{tablenotes}
  \end{threeparttable}
\end{table}

==> Tables/Parameters2.tex <==
\begin{table}[htb]
	\centering
\begin{threeparttable}
	\caption{Parameters for Simulation with URLLC flows and Med/MAcro (C-RAN) as the O-RAN scenario (see subsection \ref{subsection:O-ran}).}
           \label{Tab:Parameters2}

	\begin{tabular}{|c|c|c|}
		\hline
		Parameter & $R$ (Mbps) & $T\tnote{1}$ ($\mu$s) \\
		\hline
		vDU & 1200 & $L_{max}*8/1200$  \\
		\hline
            eth & 8000 & $L_{max}*8/8000$   \\
		\hline
		ring & 20000 & $L_{max}*8/20000$   \\
		  \hline
		\hline
		Parameter & $\rho$ (bps) & $\sigma$ (bits)\\
            \hline
		flow  & $7731\times 10^3$ & 7731 \\
		\hline
	\end{tabular}
 \begin{tablenotes}
   \item[1] This value is obtained using $T=\frac{L_{max}*8}{R}$. For URLLC, we considered a packet size of $L_{max}$=128 Bytes.  
  \end{tablenotes}
  \end{threeparttable}

\end{table}

==> Tables/ParametersCurves.tex <==
\begin{table}[htb]
    \centering
    \caption{Parâmetros utilizados para obter as curvas da Figura \ref{fig:ncb}}
        \label{tab:parameterscurves}

    \begin{tabular}{|c|c|c|c|}
    \hline
        $\rho$ & $\sigma$ & R & T\\
    \hline
    \hline

        2 & 25& 20& 10\\
        \hline
    \end{tabular}

\end{table}

==> Tables/ParametersExample.tex <==
\begin{table}[htb]
	\centering
\begin{threeparttable}
	\caption{Parameters}
   \label{Tab:ParametersExample}

	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Parameter & $R$ (Mbps) & $T\tnote{1}$ ($\mu$s) &  $\phi$ & PD ($\mu$s) \\
		\hline
		node 1 (vDU) & 50 & 40.96 &  0.5 & 0 \\
		\hline
            node 2 (eth) & 100 & 40.96 &  0.25 & 0 \\
		\hline
		node 3 (ring) & 250 & 36.384 &  0.25 & 20 \\
		\hline
		node 4 (ring) & 250 & 28.192 &  0.125 & 20 \\
		\hline
		node 5 (ring) & 250 & 24.096 &  0.0625 & 20 \\
            \hline
		\hline
		Parameter & $\rho$ (bps) & $\sigma$ (bits) &  pkt size (Bytes) & Use case \\
            \hline
		flow 1  & $1024\times 10^3$ & 1024 &  128 & URLLC \\
		\hline
		flow 2  & $512\times 10^3$ & 4096 &  128 & URLLC \\
            \hline
		flow 3  & $256\times 10^3$ & 2048 &  128  & URLLC \\
            \hline
	\end{tabular}
 \begin{tablenotes}
   \item[1] This value already takes into account PD (Propagation Delay).  
  \end{tablenotes}
  \end{threeparttable}

\end{table}

==> Tables/ProcessingDelay.tex <==
\begin{table}[htb]
\centering
 \begin{threeparttable}
	\caption{RAN Processing (adapted from 
 \cite{chun2016performance} and \cite{khatibi2018modelling})}
 	\label{tab:processingdelay}
	\begin{tabular}{|c|l|}
		\hline             \rowcolor{Gray}

		VNF & Processing (\%)   \\
		\hline
		\multirow{4}{*}{\textbf{PHY}} &  FFT: 64.99$\times$8.95=5.82\\  \cline{2-2}         
            \hline
            & Modulation: 64.99$\times$21.58=14.02\\
            \hline
            & Encoding: 64.99$\times$54.25=35.26\\
            \hline
            & Others: 64.99$\times$15.22=9.89\\   
		\hline
		MAC &  13.24\\
		\hline
		RLC &  0.91\\            \rowcolor{Gray}
		\hline
		PDCP & 18.7\\
		\hline
		RRC &  2.17\\            \rowcolor{Gray}
		\hline
		\hline
		Total & 100.01
		\hline
	\end{tabular}
  \end{threeparttable}
\end{table}

==> Tables/splitChoice5G.tex <==
\begin{table*}[htb]
\addtolength{\tabcolsep}{-2pt}
    \centering    
    \caption{Capacity and delay  requirements for different functional split options \cite{lagen2021modulation}}
        \label{tab:splitchoice5G}
    \begin{threeparttable}

    \begin{tabular}{|l|l|c|}
    \hline
         \textbf{Split}& \textbf{Capacity} & \textbf{Delay} \\
    \hline
    \hline \rowcolor{Gray}
        $O_1$ (3GPP option 1)  &   $PR \times BW/BW_{ref} \times N_L/N_{Lref} \times  M/M_{ref}$    &  10 ms           \\
        \hline
        $O_2$ (3GPP option 2-1)  & $PR \times BW/BW_{ref} \times N_L/N_{Lref} \times  M/M_{ref}$ + signaling     &  1.5-10 ms    \\
            \hline\rowcolor{Gray}
        $O_4$ (3GPP option 4)  & $PR \times BW/BW_{ref} \times N_L/N_{Lref} \times  M/M_{ref}$     & 100 $\mu$s          \\   
            \hline
        $O_6$ (3GPP option 6)  &   $(PR+CR) \times BW/BW_{ref} \times N_L/N_{Lref} \times  M/M_{ref}$     &  250 $\mu$s      \\
            \hline\rowcolor{Gray}
        $O_8$ (3GPP option 7.3) &   $(PR+CR) \times BW/BW_{ref} \times N_L/N_{Lref} \times  M/M_{ref}\times 1/cR + MAC_{info}$     &  250 $\mu$s    \\
            \hline
        $O_{9}$ (3GPP(O-RAN) option 7.2(x))  &   $N_{SC}\times N_{symb}\times W \times N_L \times 1000+MAC_{info}$     &  250 $\mu$s   \\
            \hline\rowcolor{Gray}
        $O_{11}$ (3GPP option 8) &   $SR \times W \times N_{AP} \times 5$   &  250 $\mu$s          \\
        \hline
    \end{tabular}
      \end{threeparttable}
\end{table*}

==> Tables/vivo.tex <==
\begin{table}[htb]
	\caption{Real Data from VIVO (Telefonica Brasil S.A.)}
  \label{tab:vivo}
	\centering
 \begin{threeparttable}

	\begin{tabular}{|l|l|}
            \hline 
                    MNO: VIVO (Telefonica Brasil S.A.) & Q3 2022\\
                       \hline
                        \hline \rowcolor{Gray}
            \multicolumn{2}{|c|}{Total: Mobile, Fixed \& Others} \\
		\hline
            & (millions)\\
            \hline\rowcolor{Gray}
		Net Operating Revenue & R\$ 12199 \\
		\hline
		Operational Costs &  R\$ 7242\\
		\hline\rowcolor{Gray}
		EBITDA &  R\$ 4957\\
		\hline
		D\&A &  R\$ 3226\\
		\hline\rowcolor{Gray}
		EBIT &  R\$ 1731\\
		\hline
            I\&T &  R\$ 296\\
		\hline\rowcolor{Gray}
            Net profit &  R\$ 1435\\
		\hline
\multicolumn{2}{|c|}{Mobile}\\
            \hline\rowcolor{Gray}
            & (millions)\\
            \hline
		Mobile Subscribers  & 97.328 \\
		\hline\rowcolor{Gray}
		ARPU/month &  R\$ 26.10\\
		\hline
		Net Operating Revenue &  R\$ 7621\\
  \hline\rowcolor{Gray}
  \multicolumn{2}{|c|}{Fixed}\\
            \hline
            & (millions)\\
            \hline\rowcolor{Gray}
		Mobile Subscribers  & 14.360 \\
		\hline
		ARPU/month &  R\$ 63.16\\
		\hline\rowcolor{Gray}
		Net Operating Revenue &  R\$ 2721\\
  \hline
\multicolumn{2}{|c|}{Break-Even Approach}\\  
\hline \rowcolor{Gray}           & (millions)\\
            \hline\
Mobile Operational Cost\tnote{1}& R\$ 5336\\

\hline\rowcolor{Gray}
ACPU/month\tnote{2} & R\$ 18.28\\
\hline
Mobile subscribers at BE point & 68.156\\
\hline\rowcolor{Gray}
$\zeta$ & 70.03 \%\\
\hline

	\end{tabular}
  \begin{tablenotes}
   \item[1] Simple assumption that cost is linearly proportional to revenue.
   \item[2] ACPU stands for Average Cost per User.
  \end{tablenotes}
   \end{threeparttable}
\end{table}

